On the Turing Completeness of Modern Neural Network Architectures

Alternatives to recurrent neural networks, in particular, architectures based on attention or convolutions, have been gaining momentum for processing input sequences. In spite of their relevance, the computational properties of these alternatives have not yet been fully explored. We study the computational power of two of the most paradigmatic architectures exemplifying these mechanisms: the Transformer (Vaswani et al., 2017) and the Neural GPU (Kaiser & Sutskever, 2016). We show both models to be Turing complete exclusively based on their capacity to compute and access internal dense representations of the data. In particular, neither the Transformer nor the Neural GPU requires access to an external memory to become Turing complete. Our study also reveals some minimal sets of elements needed to obtain these completeness results.

==> non_TC_residual.tex <==
We show that, with only $\hardmax$ for the attention function and with no residual connections, 
the precision of all the internal representations in the decoder of a Transformer are bounded by the precision
of its input values. They are actually bounded by $O(n\log n + nP)$ for an input of length $n$ and such that $P$ is the
maximum number of bits used for a rational number in the input.

We assume that every $v\in\sQ$ is represented by a triple $(s,n,d)\in\{1,-1\}\times\N\times\N$ such that $v=s\times\frac{n}{d}$.
We denote by $\rep(v)$ the triple representing $v$.
We denote by $\precs(v)$ the number of bits needed to store $\rep(v)$. If $\rep(v)=(s,n,d)$ then $\precs(v)$ is 
$O(\log(n)+\log(d))$.
With this representation, we only need integer summation and multiplication to simulate, summation, multiplication and
division of rationals.
Moreover notice that every basic operation over rational numbers increases its precision at most by a constant factor.
Actually, it is not difficult to see that $\precs(v_1\star v_2)$ is in $O(\precs(v_1) + \precs(v_2))=O(\precs(\max\{v_1,v_2\}))$
for every operation $\star$ among summation, multiplication and division.
Regarding computation, it is straightforward by using standard algorithms, that $\rep(v_1\star v_2)$ can be computed
from $\rep(v_1)$ and $\rep(v_2)$ with a Turing machine working in space $O(\precs(v_1) + \precs(v_2))$.

Now let $f:\Q\to\Q$ be a fixed rational function (with rational coefficients). 
Recall that a rational function is one of the form
$f(x)=P(x)/Q(x)$ where $P(x)$ and $Q(x)$ are polynomials.
Then, given that $P(x)$ and $Q(x)$ are fixed polynomials, and by the above discussion, we have that 
$\precs(f(v))$ is in $O(\precs(v))$ for every $v\in \Q$, and there is a (fixed) Turing machine $M_f$ that computes 
$\rep(f(v))$ from $\rep(v)$ in $O(\precs(v))$ space.
It is straightforward to generalize these observations to vectors. 
Given a vector $\vv=(v_1,\ldots,v_d)\in\sQ^d$ we denote by $\precs(\vv)=\precs(v_1)+\cdots+\precs(v_n)$.
Let $d$ be a fixed number, and $F:\sQ^d\to \sQ^d$
a fixed rational function, 
then $\precs(F(\vv))$ is in $O(\precs(\vv))$ and can be computed in space $O(\precs(\vv))$.

Assume that $\mX=(\vx_1,\ldots,\vx_n)\in \sQ^d$ is the input for an encoder layer $\Enc(\cdot)$ of $\Trans$.
Lets denote by $|\mX|$ the size of $\mX$. Notice that $|\mX|$ is $O(n\times \precs(\vx^\star))$ with 
$\vx^\star$ a vector such that $\precs(\vx^\star)=\max\{\precs(\vx_i)\}_{i=1}^n$.
By the discussion above, we know that $Q(\mX)$, $K(\mX)$ and $V(\mX)$ can be computed
in space $O(|\mX|)$.
Moreover, we know that every $\precs(Q(\vx_i))$, $\precs(K(\vx_i))$ and $\precs(V(\vx_i))$ is in $O(\precs(\vx^\star))$. 
Now, in order to compute $\va_i$ in Equation~(\ref{eq:enc-att}) \\ 

[*** ACA QUEDE Y SE ME FUE EN COLLERA ***]
%
%$\Att(Q(\vx_i),K(\mX),V(\mX)$ is computed as
%\[
%\Att(Q(\vx_i),K(\mX),V(\mX)=\sum_{j=1}^n\alpha_jV(\vx_j)
%\]
%\[
%\left(\sum_{j=1}^n f_{\hardmax}(\score(Q(\vx_i),K(\vx_j)))V(\vx_j)\right) \times \left(\sum_{\ell=1}^n f_{\hardmax}(\score(Q(\vx_\ell),K(\vx_\ell)))\right)^{-1}
%\]
%We now that $\score(Q(\vx_i),K(\vx_j)$ can be computed in space $O(\precs(\vx^\star))$








==> notation.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \Q^{m\times n}$ of $f: \Q^n \rightarrow \Q^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \Q
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



==> transformer_complete.tex <==

The main idea is to simulate an RNN encoder-decoder architecture
using a Transformer network. 
Let $A=(\Sigma,f,N,\vs,\sF)$ be a recognizer, with $N$ an RNN encoder-decoder 
of dimension $d$ and composed of the equations 
\begin{eqnarray*}
\vh_{i} & = & \sigma(\vx_i\mV+\vh_{i-1}\mV) \\
\vg_{t} & = & \sigma(\vg_{t-1}\mU)
\end{eqnarray*} 
with $\vh_0=\vzero$ (the vector in $\sQ^d$ with only zeros), 
and $\vg_0=\vh_n$ where $n$ is the length of the input.
%Recall that by Theorem~\ref{theo:rnn} we can also assume that $\vs=\vzero$.
We shall construct a recognizer $A'=(\Sigma,f',\Trans,\vs',\sF')$ with $\Trans$ a Transformer network such that $L(A)=L(A')$.
In our proof we will use vectors in $\sQ^{6d+8}$. 
The idea of every component of this vector will be clear when we describe the details of the construction.

\subsection*{Preliminaries}

We first introduce the embedding and positional encoding functions. 
We use an embedding function $f':\Sigma\to \sQ^{6d+8}$ such that
\[
f'(a)=[f(a),\vzero,\vzero,0,0,0,0,\vzero,\vzero,\vzero,0,0,0,0]
\]
%We use $\ve^{(i)}$ for the vector in $\sQ^{6d+8}$ with a $1$ at position $i$ and $0$ everywhere else.
Our construction uses a very simple positional encoding $\penc:\sN\to\sQ^{6d+8}$ such that $\penc(i)$ %=i\times \ve^{(6d+8)}$,
is a vector that only has the value $i$ in its last position and $0$ everywhere else.
%That is, the $i$-th symbol of a sequence shall have simply $i$ as positional encoding.
Thus if $f(a_i)=\vx_i$  we have that
\[
f_{\penc}'(a_i)=[\vx_i,\vzero,\vzero,0,0,0,0,\vzero,\vzero,\vzero,0,0,0,i]
\]
We denote this last vector by $\overline{\vx}_i$.
That is, the input for $\Trans$ is the sequence $(\overline{\vx}_1,\overline{\vx}_2,\ldots,\overline{\vx}_n)$.
We need a final notation to begin with the proof. We will usually have the last component
of all our vectors with the positional encoding. 
Thus, given an arbitrary vector $\vv\in \sQ^{6d+8}$ we denote by $e(\vv)$ the value of its last
component. That is, for the vector $\overline{\vx}_i$ above we have $e(\overline{\vx}_i)=i$.

\subsection*{The attention mechanism used}

In what follows we will use a scoring function $\score:\sQ^{6d+8}\times \sQ^{6d+8}\to \sQ$ that essentially
performs the following computation for a pair of vectors $(\vq,\vk)$:
\[
\score(\vq,\vk) = 
-|e(\vq) - e(\vk)|
\]
This function can be implemented with an additive attention as follows.
We use a feed-forward network of three layers that receives as input a vector of the form $[\vq,\vk]\in \sQ^{2(6d+8)}$.
The first layer will be a function $f_1:\sQ^{2(6d+8)}\to \sQ^2$ that just picks the values at positions
$6d+8$ and at $2(6d+8)$, thus, with input $[\vq,\vk]$ it produces $f_1([\vq,\vk])=[e(\vq),e(\vk)]$.
It is clear that this transformation can be performed with a single-layer neural network (with an identity activation) 
since this is just a linear transformation. The next two layers are defined by functions $f_2:\sQ^2\to \sQ^2$, 
and $f_3:\sQ^2\to \sQ$ defined as follows:
\begin{eqnarray*}
f_2([x,y]) & = & \relu([x-y, y-x]) \\
f_3([x,y)] & = & - x - y
\end{eqnarray*}
Thus, $\score(\vq,\vk)$ will be
\[
\score(\vq,\vk) = f_3(f_2(f_1([\vq,\vk])))
\]
It is not difficult to see that the result will be
\[ 
\score(\vq,\vk)=-\relu(e(\vq)-e(\vk))-\relu(e(\vk)-e(\vq)) = -|e(\vq)-e(\vk)| 
\]
which is exactly what we wanted to obtain.

%
%\[f_1(\vz) = \mA_1\vz = 
%\left[
%\begin{array}{c}
%\vz_{6d+8} \\
%\vz_{2(6d+8)}
%\end{array}
%\right]
%\]
%
%where $\mA_1 = [\vzero,\ve^{(6d+8)};]$ and this vectors are of size $8d+18$.
%
%\[f_2(\vz) = \left[ \begin{array}{ccc}
%1 & -1 \\
%-1 & 1 \\
%\end{array} \right] \vz \]
%
%\[f_3(\vz) = relu(\vz) \]
%
%\[f_4(\vz) = [-1,-1]\vz \]
%
%The $NN$ is defined for vectors of size $8d+18$, and is defined by the recurrence $\vz_i = 
%f_i(\vz_{i-1})$, with $\vz_0$ being the input to the network and $\vz_4$ its output.
%
%Notice that the previous network acting over $[\vq;\vk]$ has the following effect:
%
%\[ [\vq;\vk] \rightarrow [e(\vq);e(\vk)] \rightarrow [e(\vq)-e(\vk);e(\vk)-e(\vq)] \rightarrow 
%relu([e(\vq)-e(\vk);e(\vk)-e(\vq)]) \rightarrow \]
%\[ -relu(e(\vq)-e(\vk))-relu(e(\vk)-e(\vq)) = -|e(\vq)-e(\vk)| \]
%
%For the embedding, we shall use $f(\vx) = [\vzero;\vx;\vzero;0]$.

The most important property of this score function is that, when combined with hard attention, it has
the effect of attending to a specific position of the attended sequence of vectors. 
More formally, assume that $\vq$ is a vector such that $1\leq e(\vq)\leq n$,
and $\vk_1,\vk_2,\ldots,\vk_n$ are all such that $e(\vk_i)=i$.
Then we have that the following holds:
\begin{eqnarray*}
(\score(\vq,\vk_1),\score(\vq,\vk_2),\ldots,\score(\vq,\vk_n)) & = & (-k, -k+1, \ldots, -1,0,-1,\ldots, -(n-k))
\end{eqnarray*}
where the $0$ appears exactly in the $k$-th position of the above vector.
Thus we have that
\begin{eqnarray*}
\hardmax(\score(\vq,\vk_1),\score(\vq,\vk_2),\ldots,\score(\vq,\vk_n)) & = & (0,0,\ldots,0,1,0,\ldots,0)
\end{eqnarray*}
Where the $1$ appears exactly in the $k$-th position.
Moreover, if we assume that $e(\vq)=k$ such that $k>n$ then
\begin{eqnarray*}
(\score(\vq,\vk_1),\score(\vq,\vk_2),\ldots,\score(\vq,\vk_n)) & = & (-k, -k+1, \ldots,  -k+n)
\end{eqnarray*}
and thus the maximum value occurs in the last position which implies that
\begin{eqnarray*}
\hardmax(\score(\vq,\vk_1),\score(\vq,\vk_2),\ldots,\score(\vq,\vk_n)) & = & (0,0,\ldots,0,1)
\end{eqnarray*}
That is, it is the sequence with a $1$ in its last position.

%just taking one vector from the attended sequence,
%the one whose key has encoding value nearest to the value of the
%query, ignoring the rest.
Putting all this in the $\Att$ function, we obtain the following. 
Assume that we have a sequence $\mK=(\vk_1,\ldots,\vk_n)$ of key vectors such that
$e(\vk_i)=i$ for every $i$.
Let $\mV=(\vv_1,\ldots,\vv_n)$ be a sequence of arbitrary value vectors, 
and assume that we have a query $\vq$ such 
that $1\leq e(\vq) \leq n$. Then we have
\[
\Att(\vq,\mK,\mV)=\vv_{e(\vq)}.
\]
Moreover, whenever we have a query vector $\vq$ such that $e(\vq)>n$ then
\[
\Att(\vq,\mK,\mV)=\vv_n.
\]
Given this property and also given that all vectors that we use will have a positional encoding in its last component,
to simplify the notation we can use the function $\Att(i,\mK,\mV)=\vv_i$, and thus
\[
\Att(\vq,\mK,\mV)=\Att(e(\vq),\mK,\mV)
\]
Notice that
\[
\Att(i,\mK,\mV)=
\begin{cases}
\vv_i & i \leq n \\
\vv_n & i > n
\end{cases}
\]
We extensively use these properties of the attention function in our construction.
We now have all the necessary to begin with the details of our proof.

\subsubsection*{Construction of $\TEnc$}

The encoder part of $\Trans$ is very simple. For $\TEnc$ we use a single-layer encoder, 
such that $\TEnc(\overline{\vx}_1,\ldots,\overline{\vx}_n)=(\mK^{\ve},\mV^{\ve})$ where
\[
\mK^{\ve} = (\overline{\vx}_1,\ldots,\overline{\vx}_n)
\]
that is, it implements the identity function for keys, and
\[
\mV^{\ve} = (\overline{\vv}_1,\ldots,\overline{\vv}_n)
\]
where
\[
\overline{\vv}_i = [\vx_i,\vzero,\vzero,0,0,0,i,\vzero,\vzero,\vzero,0,0,0,0]
\]
That is, $\overline{\vv}_i$ is just $\overline{\vx}_i$ where the last component has been moved to the center component.
It is straightforward that this can be done with a single layer encoder by just implementing the identity
(that can be done by taking advantage of the residual connection in Equations~(\ref{eq:enc-att}) and~(\ref{eq:enc-out})),
and then using affine transformations for $V(\cdot)$ and $K(\cdot)$ in Equation~(\ref{eq:enc-rec}).
The most important part of the construction is in the decoder that we next describe.

\subsection*{Overview of the contruction of $\TDec$}

\newcommand{\valpha}{\bm{\alpha}}
\newcommand{\vbeta}{\bm{\beta}}
\newcommand{\vgamma}{\bm{\gamma}}

We base our proof in the construction the following sequences of vectors and values:
\begin{eqnarray*}
\valpha_i & = & \begin{cases} 
\vx_i & 1 \leq i \leq n \\
\vx_n & i > n
\end{cases} \\
\vbeta_i & = & \begin{cases} 
\vh_i & 0 \leq i \leq n \\
\sigma(\vbeta_{i-1}\mW + \valpha_i\mV) & i > n
\end{cases} \\
\vgamma_i & = & \begin{cases}
\vzero & i \leq n \\
\vbeta_{n} & i = n+1 \\
\sigma(\vgamma_{i-1}\mU) & i > n+1
\end{cases} \\
a_i & = & \begin{cases} 
0 & 0 \leq i \leq n \\
1 & i > n
\end{cases} \\
b_i & = & \begin{cases} 
0 & i = n+1 \\
1 & i \neq n+1
\end{cases} \\
c_i & = & \begin{cases} 
i & 0 \leq i \leq n \\
n & i > n 
\end{cases} 
\end{eqnarray*}

%\[
%\vx_i' = \begin{cases} 
%\vx_i & 1 \leq i \leq n \\
%\vx_n & i > n
%\end{cases}
%\]
%\[ \vh_i' = \sigma(\mW\vh_{i-1}' + \mV\vx_i') \]
%\[ a_i = [i \geq n] \]
%\[ b_i = [i = n] \]
%\[ c_i = \begin{cases} 
%i & 1 \leq i \leq n \\
%n & i > n
%\end{cases}\]
%\[\vg_i' = \sigma(\mU\vg_{i-1}'')\]
%\[\vg_i'' = \vg_i' + b_i\vh_{i-1})\]￼
%

It is easy to see that since $\vbeta_0 = \vh_0$ and 
$\valpha_i = \vx_i$ for $1 \leq i \leq n$, then $\vbeta$ follows the recurrence 
$\vbeta_i = \sigma(\vbeta_{i-1}\mW + \vx_i\mV)$ with the same starting value and equations as the $\vh_i$'s
, and so we have that $\vbeta_i = \vh_i$ for $i \leq n$.
Then, since $\vgamma_{n+1} = \vbeta_n = \vh_n = \vg_0$, and after that 
$\vgamma_{i} = \sigma(\mU\vgamma_{i-1})$, we conclude that $\vgamma_{n+1+i}=\vg_i$.
We will show that these sequences can be computed in a transformer network,
and so we can simulate the RNN $N$.

In what follows we show an overview on how to compute all these sequences with the decoder part of $\Trans$. 
%\[
%Q(\overline{\vx}_i)=K(\overline{\vx}_i)=\overline{\vx}_i %[\vzero,\vzero,\vzero,0,0,0,0,\vzero,\vzero,0,0,0,i]
%\]
%Denoting by $att(i)$ as the value obtained
%by attending over the encoder output with a vector with encoding value $i$,
%$att_{\vx}(i)$ the $\vx$ part of $att(i)$ and $att_e(i)$ for the encoding part.
In the decoder, we show how to produce the sequence of outputs $(\vy_1,\vy_2,\ldots,\vy_r)$
where $\vy_i$ is given by:
\[ 
\vy_i = [\vzero,\vbeta_i,\vgamma_i,a_i,b_i,c_i,0,\vzero,\vzero,\vzero,0,0,0,0] \]
%\[ \vy_i = [\vh_i';\vg_i';a_i;b_i;c_i;\vzero;0;\vzero;\vzero;0;0;
%0;i+1] \]
We consider as the starting vector for the decoder the vector
\[
\vy_0 = [\vzero,\vzero,\vzero,0,1,0,0,\vzero,\vzero,\vzero,0,0,0,0].
\]
Thus,  what we are actually stating is that $\vbeta_0=\vgamma_0=\vzero$, $a_0=c_0=0$ and $b_0=1$, which
coincide with the values for the sequences described above. 
Recall that we are using positional encodings, thus, when producing the output,
the actual input for the first layer of the decoder will be the sequence
\[
\vy_0+\penc(1), \vy_1+\penc(2), \ldots, \vy_{r}+\penc(r+1)
\]
We denote by $\overline{\vy}_i$ the vector $\vy_i$ plus its positional encoding (which is always at its last component).

We now roughly describe a two-layer decoder network that, with input $\mK^{\ve},\mV^{\ve}$ and sequence $(\overline{\vy}_0,\ldots,\overline{\vy}_r)$ will produce
$\vy_{r+1}$ as output (the details are in the following section).
Our construction will resemble a proof by induction; we show how to construct $\vy_{r+1}$ from the previous vector $\vy_r$.

%We now proceed to describe the decoder part of the Transformer that only uses two layers.
The overview of the construction is very simple. 
With input $\mK^{\ve},\mV^{\ve}$ and sequence $(\overline{\vy}_0,\ldots,\overline{\vy}_r)$
the first decoder layer produces a sequence of vectors $\vz_0^1,\vz_1^1,\ldots, \vz_{r}^1$ such that
\begin{equation}\label{eq:first-layer}
\vz^1_{i} = [\valpha_{i+1},\vbeta_i,\vgamma_i,a_i,b_i,c_i,c_{i+1},\vbeta_{i+1},\vgamma_{i+1},\vzero,a_{i+1},b_{i+1},c_{i+1},i+1]
\end{equation}
Notice that the first decoder layer will do almost all the heavy work. 
We actually use a feed-forward network with 3 layers to obtain this output.
After that,  the second decoder layer, just do some cleaning work by moving
some parts of the vector and deleting others to produce the sequence of output vectors $\vz_0^2,\vz_1^2,\ldots, \vz_{r}^2$ where
\begin{equation}\label{eq:second-layer}
\vz^2_{i}=[\vzero,\vbeta_{i+1},\vgamma_{i+1},a_{i+1},b_{i+1},c_{i+1},0,\vzero,\vzero,\vzero,0,0,0,0].
\end{equation}
This is exactly what we want as output, and thus, we just consider the final output transformation $F(\cdot)$
as the identity to produce $\vy_{r+1}=F(\vz_r^2)$ (Equation~(\ref{eq:dec-out})) which completes our construction.


\subsection*{Detailed construction of $\TDec$}
First, we have the following useful identities for $\valpha_i$, $\vbeta_i$ and $\vgamma_i$ 
that can be obtained by simply inspecting the definitions above and the attention
function that we defined:
\begin{eqnarray*}
\valpha_i & = & \Att(i,\mK^{\ve},\mV^{\ve})_{1:d} \\
\vbeta_i & = & \begin{cases} 
\vzero & i = 0 \\
\sigma(\vbeta_{i-1}\mW + \valpha_i\mV) & i > 0
\end{cases} \\
\vgamma_i & = & \begin{cases}
\vzero & i = 0 \\ 
\sigmoid(\vgamma_{i-1}\mU) + (1-b_i)\vbeta_{i-1} & i > 0
\end{cases}
\end{eqnarray*}
We also have some identities for $a_i$, $b_i$ and $c_i$:
\begin{eqnarray*}
c_i & = &  \begin{cases}
0 & i = 0 \\
\Att(i,\mK^{\ve},\mV^{\ve})_{3d+4} & i > 0
\end{cases} \\
a_i & = & \begin{cases}
0 & i = 0 \\
1-(c_i-c_{i-1}) & i > 0
\end{cases} \\
b_i & = & \begin{cases}
1 & i = 0 \\
1-(a_i-a_{i-1}) & i > 0
\end{cases} 
\end{eqnarray*}
%where $(\valpha_i)_{3d+4}$ is the element at position $3d+4$ in $\valpha_i$.
We also note that $b_i$ can be rewritten as:
\begin{eqnarray*}
b_i & = & \begin{cases}
1 & i = 0 \\
c_i-c_{i-1}+a_{i-1} & i > 0
\end{cases}
\end{eqnarray*}
%\[ \vx_i' = att(i)_{\vx} \]
%\[ c_i = att(i)_e, c_0 = 0 \]
%\[ a_i = 1-(c_i-c_{i-1}) \]
%\[ b_i = 1-(a_i-a_{i-1}) = 1-(1-(c_i-c_{i-1})-a_{i-1}) = c_i-c_{i-1}+a_{i-1})\]
%\[ b_i\vh_{i-1} = \sigma(\vh_{i-1}-b_i)\]
%These identities can be used to compute $\vy_{i+1}$ from $\vy_i$￼￼.


The first layer of the decoder, that we call $\Dec_1$, is defined by the functions $Q_1(\cdot)$, $V_1(\cdot)$, $K_1(\cdot)$,
and $O_1(\cdot)$ that we now describe.
We use the function $V_1:\sQ^{6d+8}\to \sQ^{6d+8}$ such that $V_1(\vv)$ is the vector with only zeroes, 
thus, we just \emph{nullify} the self-attention in the first decoder layer.
This plus the residual connection in Equation~(\ref{eq:dec-self}) has the net effect of producing the identity
and thus we obtain $\vp_{i}^1=\overline{\vy}_{i}$ for every $i\in \{0,\ldots,r\}$.
Notice that $e(\vp_{i}^1)=e(\overline{\vy}_{i})=i+1$, and thus, if $i+1\leq n$ we have that
\[
\Att(\vp_i^1,\mK^{\ve},\mV^{\ve})=\Att(i+1,\mK^{\ve},\mV^{\ve})=\overline{\vv}_{i+1} = [\vx_{i+1},\vzero,\vzero,0,0,0,i+1,\vzero,\vzero,\vzero,0,0,0,0]
\]
and, otherwise, if $i+1>n$ we have
\[
\Att(\vp_i^1,\mK^{\ve},\mV^{\ve})=\Att(i+1,\mK^{\ve},\mV^{\ve})=\overline{\vv}_{n} = [\vx_{n},\vzero,\vzero,0,0,0,n,\vzero,\vzero,\vzero,0,0,0,0].
\]
Thus, combining both cases we actually have that
\[
\Att(\vp_i^1,\mK^{\ve},\mV^{\ve})=[\valpha_{i+1},\vzero,\vzero,0,0,0,c_{i+1},\vzero,\vzero,\vzero,0,0,0,0].
\]
This last result is summed with $\vp_i^1=\overline{\vy}_{i}$ (the residual connection in Equation~(\ref{eq:dec-ext})) 
to obtain $\va^1_{i}$ which is given by:
\begin{eqnarray*}
\va_i^1 & = & \Att(\vp_i^1,\mK^{\ve},\mV^{\ve})+\vp_i^1 \\
& = & [\valpha_{i+1},\vbeta_i,\vgamma_i,a_i,b_i,c_i,c_{i+1},\vzero,\vzero,\vzero,0,0,0,i+1]
\end{eqnarray*}
We now describe the function $O_1(\cdot)$ which is going to be defined by a feed-forward neural network that
we next describe.
The first layer of the network will be given by a function $f_1:\sQ^{6d+8}\to \sQ^{6d+8}$ such that
with input $\va_i^1$ it will produce
\[ 
f_1(\va_i^1)= [\valpha_{i+1},\vbeta_i,\vgamma_i,0,0,0,0,\vzero,\vzero,\vzero,a_{i+1},b_{i+1},0,0].
\]
It is clear that $f_1$ can be implemented with a single neural-network layer as it only has to apply the
affine transformation given by the equations
$a_{i+1}=1-(c_{i+1}-c_i)$ and $b_{i+1}=c_{i+1}-c_i+a_i$, and making some positions equal to $0$.

After $f_1$ we apply another feed-forward layer $f_2:\sQ^{6d+8}\to \sQ^{6d+8}$ given by
\begin{eqnarray*}
f_2(f_1(\va_i^1)) & = & \sigmoid([\vzero,\vbeta_i,\vgamma_i,0,0,0,0,\vbeta_i\mW+\valpha_{i+1}\mV,\vgamma_i\mU,\vbeta_i-b_{i+1}\bm{1},a_{i+1},b_{i+1},0,0])
\end{eqnarray*}
where $\bm{1}$ is a vector in $\sQ^d$ with only ones. 
It is clear that the internal vector can be computed with an affine transformation.
Since $a_{i+1},b_{i+1}$ are all rationals between $0$ and $1$,
and all the values in $\vbeta_i$ and $\vgamma_i$ are also between $0$ and $1$, when we apply the function $\sigmoid$ we obtain
\begin{equation*}
f_2(f_1(\va_i^1)) = 
[\vzero,\vbeta_i,\vgamma_i,0,0,0,0,\sigmoid(\vbeta_i\mW+\valpha_{i+1}\mV),\sigmoid(\vgamma_i\mU),\sigma(\vbeta_i-b_{i+1}\bm{1}),a_{i+1},b_{i+1},0,0]). \\
\end{equation*}

We note that $\sigmoid(\vbeta_i\mW+\valpha_{i+1}\mV)$ is actually $\vbeta_{i+1}$.
Moreover, as we next describe, it holds that $\sigma(\vbeta_i-b_{i+1}\bm{1})=(1-b_{i+1})\vbeta_i$.
To see this, notice that $\vbeta_i$ has all its values between $0$ and $1$.
Then, if $b_{i+1}=1$ we have that $\vbeta_i-b_{i+1}\bm{1}$ is a vector with all its components less than
or equal to $0$ which implies that $\sigmoid(\vbeta_i-b_{i+1}\bm{1})=\vzero$. On the other hand, 
if $b_{i+1}=0$ then $\sigmoid(\vbeta_i-b_{i+1}\bm{1})=\sigmoid(\vbeta_i)=\vbeta_i$.
Thus we can write the output of this layer as:
\begin{eqnarray*}
f_2(f_1(\va_i^1)) & = & 
[\vzero,\vbeta_i,\vgamma_i,0,0,0,0,\vbeta_{i+1},\sigmoid(\vgamma_i\mU),(1-b_{i+1})\vbeta_i,a_{i+1},b_{i+1},0,0]). 
\end{eqnarray*}
We need a final linear layer given by a function $f_3:\sQ^{6d+8}\to \sQ^{6d+8}$ 
that does the following computation
\begin{eqnarray*}
f_3(f_2(f_1(\va_i^1))) & = & 
[\vzero,\vzero,\vzero,0,0,0,0,\vbeta_{i+1},\sigmoid(\vgamma_i\mU)+(1-b_{i+1})\vbeta_i,\vzero,a_{i+1},b_{i+1},0,0]). 
\end{eqnarray*}
Notice that $\sigmoid(\vgamma_i\mU)+(1-b_{i+1})\vbeta_i$ is exactly $\vgamma_{i+1}$ thus the output of $f_3$ can be written as
\begin{eqnarray*}
f_3(f_2(f_1(\va_i^1))) & = & 
[\vzero,\vzero,\vzero,0,0,0,0,\vbeta_{i+1},\vgamma_{i+1},\vzero,a_{i+1},b_{i+1},0,0]). 
\end{eqnarray*}
This is the output of function $O_1(\cdot)$. Thus. we have that
\begin{eqnarray*}
O_1(\va_i^1) & = & f_3(f_2(f_1(\va_i^1))) \\
 & = & 
[\vzero,\vzero,\vzero,0,0,0,0,\vbeta_{i+1},\vgamma_{i+1},\vzero,a_{i+1},b_{i+1},0,0]). 
\end{eqnarray*}
Now the output of this decoder layer is $\vz_i^1=O_1(\va_i^1)+\va_i^1$ (Equation~(\ref{eq:dec-ff})) and thus we have
\begin{eqnarray*}
\vz_i^1 & = & O_1(\va_i^1) + \va_i^1 \\
 & = & 
[\valpha_{i+1},\vbeta_i,\vgamma_i,a_i,b_i,c_i,c_{i+1},\vbeta_{i+1},\vgamma_{i+1},\vzero,a_{i+1},b_{i+1},0,i+1]). 
\end{eqnarray*}

For the second decoder layer $\Dec_2$, it is straightforward to construct a layer that just do some cleaning and thus
from $\vz_0^1,\vz_1^1,\ldots, \vz_r^1$ produces the sequence $\vz_0^2,\vz_1^2,\ldots, \vz_r^2$ such that
\begin{eqnarray*}
\vz_i^2 & = & 
[\vzero,\vbeta_{i+1},\vgamma_{i+1},a_{i+1},b_{i+1},c_{i+1},0,\vzero,\vzero,\vzero,0,0,0,0]). 
\end{eqnarray*}
We finally use $F(\cdot)$ as the identity function to produce our desired output from $\vz_r^2$, that is
\[
\vy_{r+1} = F(\vz_r^2)  = [\vzero,\vbeta_{r+1},\vgamma_{r+1},a_{r+1},b_{r+1},c_{r+1},0,\vzero,\vzero,\vzero,0,0,0,0]). 
\]
This completes the construction and the correctness of our construction.

\subsection*{Final step}
We now can use our $\Trans$ network to construct the recognizer $A'=(\Sigma,f',\Trans,\vs',\sF')$.
We use $\vs'$ as simple $\vy_0$ in our above construction.
Finally, notice that in $\Trans$ the vector $\vgamma_i$ is actually the output of the RNN encoder-decoder 
that we are simulating but only for $i\geq n+1$. 
We take advantage of the value $a_{i}$ which is $1$ if and only if $i\geq n+1$.
Thus we can define $\sF'=\sQ^{2d}\times \sF\times \{1\}\times \sQ^{3d+7}$.
This completes the proof of the Theorem.


